Independent Component Alignment for Multi-Task Learning

In a multi-task learning (MTL) setting, a single model is trained to tackle a diverse set of tasks jointly. Despite rapid progress in the field, MTL remains challenging due to optimization issues such as conflicting and dominating gradients. In this work, we propose using a condition number of a linear system of gradients as a stability criterion of an MTL optimization. We theoretically demonstrate that a condition number reflects the aforementioned optimization issues. Accordingly, we present Aligned-MTL, a novel MTL optimization approach based on the proposed criterion, that eliminates instability in the training process by aligning the orthogonal components of the linear system of gradients. While many recent MTL approaches guarantee convergence to a minimum, task trade-offs cannot be specified in advance. In contrast, Aligned-MTL provably converges to an optimal point with pre-defined task-specific weights, which provides more control over the optimization result. Through experiments, we show that the proposed approach consistently improves performance on a diverse set of MTL benchmarks, including semantic and instance segmentation, depth estimation, surface normal estimation, and reinforcement learning. The source code is publicly available at https://github.com/SamsungLabs/MTL .

==> figs/tikz/main_first.tex <==
% \begin{document}
\begin{tikzpicture}%[font=\LARGE] 

\coordinate (OLD_L1)    at ({-4.8}, {1.48)});
\coordinate (OLD_L2)    at ({4.89}, {4.99)});
\coordinate (NEW_L1)    at ({-3.42}, {3.68});
\coordinate (NEW_L2)    at ({6.73}, {1.87)});
\coordinate (RO_L1)    at ({-2.4}, {0.74});
\coordinate (RO_L2)    at ({2.445}, {2.495)});
\coordinate (O)         at (0,0);




\draw[dashed,-stealth, red] (O)--(NEW_L1); % x axis
\draw[dashed,-stealth, blue] (O)--(NEW_L2); % y axis
\draw[thin, ->] (RO_L1) arc (160:130:2.51) node[above right] {$U^\top$};
\draw[thin, ->] (RO_L2) arc (50:20:3.5) node[below right] {$U^\top$};
\draw[ultra thick,-stealth, red] (O)--(OLD_L1) node[above right] {$\nabla\mathcal{L}^1$}; % old grad1
\draw[ultra thick,-stealth, blue] (O)--(OLD_L2) node[above] {$\nabla\mathcal{L}^2$}; % old grad2


\end{tikzpicture}
% \end{document}

==> figs/tikz/main_fourth.tex <==
% \documentclass[tikz,border=10pt]{standalone}
% \usepackage{tkz-euclide}

% \begin{document}
\begin{tikzpicture}%[font=\LARGE] 

% Bounding box
% \path (-1,-1.3) rectangle (4.5,2.9);

\definecolor{darkgreen}{RGB}{255,51,76}


\coordinate (OLD_L1)    at ({-4.8}, {1.48)});
\coordinate (OLD_L2)    at ({4.89}, {4.99)});
\coordinate (NEW_L1)    at ({-3.464}, {2.254});
\coordinate (NEW_L2)    at ({2.254}, {3.464)});
\coordinate (L1_L2)    at ({-0.605}, {2.859)});
\coordinate (RO_L1)    at ({-0.9365}, {1.842});
\coordinate (RO_L2)    at ({1.842}, {0.9365)});
\coordinate (O)         at (0,0);
% \coordinate (OX)        at (8, 0);
% \coordinate (OY)        at (0, 5);




\draw[ultra thick,-stealth, red] (O)--(NEW_L1) node[above right,xshift=-1em] {$\nabla\mathcal{L}^1_\text{new}$}; 
\draw[ultra thick,-stealth, blue] (O)--(NEW_L2) node[above] {$\nabla\mathcal{L}^2_\text{new}$};
\draw[ultra thick,-stealth, black!60!green] (O)--(L1_L2) node[above,yshift=2em,xshift=-3em] {$w_1\nabla\mathcal{L}^1_\text{new} {+} w_2\nabla\mathcal{L}^1_\text{new}$};
\draw[dashed,-stealth, red] (O)--(OLD_L1) node[above left,xshift=2em] {$\nabla\mathcal{L}^1_\text{old}$}; 
\draw[dashed,-stealth, blue] (O)--(OLD_L2) node[above right,yshift=-3em,xshift=-1em] {$\nabla\mathcal{L}^2_\text{old}$}; 
\tkzMarkRightAngle(NEW_L1,O,NEW_L2)

\end{tikzpicture}
% \end{document}

==> figs/tikz/main_second.tex <==
\begin{tikzpicture}%[font=\LARGE] 

% Bounding box
% \path (-1,-1.3) rectangle (4.5,2.9);

\coordinate (NEW_L1)    at ({-1.873}, {3.684)});
\coordinate (NEW_L2)    at ({3.684}, {1.873)});
\coordinate (OLD_L1)    at ({-3.42}, {3.68});
\coordinate (OLD_L2)    at ({6.73}, {1.87)});
\coordinate (RO_L1)    at ({-1.71}, {1.84});
\coordinate (RO_L2)    at ({3.365}, {0.935)});
\coordinate (O)         at (0,0);
\coordinate (OX)        at (8, 0);
\coordinate (OY)        at (0, 5);




\draw[dashed,-stealth, red] (O)--(NEW_L1); 
\draw[dashed,-stealth, blue] (O)--(NEW_L2);
\draw[ultra thick,-stealth, red] (O)--(OLD_L1) node[above right] {$\nabla\mathcal{L}^1$}; 
\draw[ultra thick,-stealth, blue] (O)--(OLD_L2) node[above right] {$\nabla\mathcal{L}^2$}; 
\draw[thin, ->] (RO_L1) arc (135:120:2.51) node[above right] {$\Sigma^{-1}$};
\draw[thin, ->] (RO_L2) arc (20:31:3.5) node[above left] {$\Sigma^{-1}$};
\tkzMarkRightAngle(NEW_L1,O,NEW_L2)



\end{tikzpicture}
% \end{document}

==> figs/tikz/main_third.tex <==
% \documentclass[tikz,border=10pt]{standalone}
% \usepackage{tkz-euclide}

% \begin{document}
\begin{tikzpicture}%[font=\LARGE] 

% Bounding box
% \path (-1,-1.3) rectangle (4.5,2.9);


\coordinate (OLD_L1)    at ({-1.873}, {3.684)});
\coordinate (OLD_L2)    at ({3.684}, {1.873)});
\coordinate (NEW_L1)    at ({-3.464}, {2.254});
\coordinate (NEW_L2)    at ({2.254}, {3.464)});
\coordinate (RO_L1)    at ({-0.9365}, {1.842});
\coordinate (RO_L2)    at ({1.842}, {0.9365)});
\coordinate (O)         at (0,0);
% \coordinate (OX)        at (8, 0);
% \coordinate (OY)        at (0, 5);




\draw[dashed,-stealth, red] (O)--(NEW_L1); 
\draw[dashed,-stealth, blue] (O)--(NEW_L2);
\draw[ultra thick,-stealth, red] (O)--(OLD_L1) node[above right] {$\nabla\mathcal{L}^1$}; 
\draw[ultra thick,-stealth, blue] (O)--(OLD_L2) node[above right] {$\nabla\mathcal{L}^2$}; 
\draw[thin, ->] (RO_L1) arc (120:149:2.066) node[below left] {$U$};
\draw[thin, ->] (RO_L2) arc (20:50:2.066) node[above left] {$U$};
\tkzMarkRightAngle(OLD_L1,O,OLD_L2)

\end{tikzpicture}
% \end{document}

==> figs/toy_1a_teaser.tex <==
\begin{figure}[t!]
\centering

\begin{subfigure}[t]{.23\textwidth}
  \centering
  \includegraphics[width=1.0\textwidth]{./figs/pictures/toy_1a/3d-obj.pdf}
\end{subfigure}
\hfill
\begin{subfigure}[t]{.23\textwidth}
  \centering
  \includegraphics[width=1.0\textwidth]{./figs/pictures/toy_1a/contours.png}
\end{subfigure}
\hfill
\begin{subfigure}[t]{.23\textwidth}
  \centering%\tiny
  \includegraphics[width=1.0\textwidth]{./figs/pictures/toy_1a/loss_pnt0.pdf}
  %\caption{IMTL~\cite{liu2021_imtl}}
\end{subfigure}
\hfill
\begin{subfigure}[t]{.23\textwidth}
  \centering
  \includegraphics[width=1.0\textwidth]{./figs/pictures/toy_1a/loss_pnt2.pdf}
\end{subfigure}

\caption{Following~\cite{tianhe2020pcgrad}, we evaluate our approach and other MTL methods on an optimization problem $\mathcal{L}_0$ consisting of two tasks (upper left). For each MTL approach, we visualize convergence curves starting from two initial points: $P_0$ (bottom left) and $P_2$ (bottom right). Clearly, aligned-MTL is stable and converges faster to a global minimum. More details can be found in~\cref{ssec:synthetic_mtl_problem}.}
 \label{fig:teaser}
\end{figure}

% Following [59], we evaluate our approach and recent gradient manipulation MTL methods
%on an optimization problem consisting of 2 tasks (denoted by ?). For each MTL method, we visualize
%the trajectory steps (from red to orange) of gradient updates computed from 3 different initial points •.
%MGDA and PCGrad stop optimization once they attain the Pareto set converging to a poor
%Pareto-stationary point. The proposed method converges faster to a global minimum (subplots d–e)
%by reducing fluctuations in conflict regions. See Sec. 7.1 for more details.

==> figs/toy_1c.tex <==
\begin{figure}[t!]
%   \huge
  \centering
  \def\scale{.17}
%   \tikzset{every picture/.style={line width=3pt}}
  \begin{subfigure}[t]{0.24\textwidth}  
    \centering
    \includegraphics[scale=0.5]{./figs/pictures/toy_1c/loss_0.pdf}
        % \includesvg{./figs/pictures/method/stage_1.svg}
        %\input{./figs/tikz/main_first}
    
    % \caption{Compute SVD}
    % \label{fig:three-a}    
  \end{subfigure}
  \hfill
  \begin{subfigure}[t]{0.24\textwidth}    
    \centering
    \includegraphics[scale=0.5]{./figs/pictures/toy_1c/loss_1.pdf}
        % \includesvg{./figs/pictures/method/stage_2.svg}
        % \input{./figs/tikz/main_second} 
    % \caption{Align Principal Axes}    
    % \label{fig:three-b}    
  \end{subfigure}    

  \caption{\textbf{Geometric interpretation} of the proposed method. (a)~Initial rotation induced by an orthogonal matrix $\mU$. (b)~Scaling space along independent directions. (c)~Rotation back to an initial basis. (d)~Transformed gradients are then summed up with pre-defined tasks weights $\vw$, which gives an accumulated gradient.}
  \label{fig:amgda_geometric}
\end{figure}

==> latexmkrc <==
add_cus_dep( 'tex', 'aux', 0, 'makeexternaldocument' );

sub makeexternaldocument {
    # if the dependency isn't one of the files that this latexmk run will consider, process it
    # without this test, we would get an infinite loop!
    if (!($root_filename eq $_[0]))
    {   # PLEASE ENABLE ONLY ONE OF THE FOLLOWING
        # DEPENDING ON THE ENGINE YOU'RE USING
    
        # FOR PDFLATEX
        system( "latexmk -pdf \"$_[0]\"" );

        # FOR LATEX+DVIPDF
        # system( "latexmk \"$_[0]\"" );

        # FOR XELATEX
        # system( "latexmk -xelatex \"$_[0]\"" );
        
        # FOR LUALATEX
        # system( "latexmk -lualatex \"$_[0]\"" );
   }
}


==> tables/relocalization.tex <==
%\sisetup{round-mode=places, round-precision=2, detect-weight=true,detect-inline-weight=math}

\begin{table*}[t!] 
\caption{Camera relocalization performance of the proposed method and existing MTL approaches for the \textsc{7scenes} data set. For each scene we highlight the best performing method in terms of translation and orientation error in \protect\tikz[baseline=-.45ex]\protect\node[fill=mygray,inner sep=2pt,rounded corners=1pt]{gray};. We report median translation~$\vt$, orientation~$\vr$ errors and the growth rate, $\mathcal{R}$ for each scene. The proposed A-MGDA-UB approach can consistently improve both orientation and translation localization performance.
}
%\begin{subtable}[t]{\textwidth}
    \centering\scriptsize
    \renewcommand{\tabcolsep}{3pt}
    \begin{tabular}{l| c c c c c c c | c c}
    \toprule
    & \multicolumn{7}{c}{Scenes (error~[$m/^{\circ}$]~$\downarrow$)} & & \\
    {Method} & \textsc{chess} & \textsc{fire} & \textsc{heads} & \textsc{office} & \textsc{pumpkin} & \textsc{kitchen} & \textsc{stairs} & {Average} & {$\mathcal{R}$~[\%]~$\uparrow$} \\
    \midrule
  Baseline: Uniform & $0.17/8.44$ & $0.63/11.10$ & $1.81/13.12$ & $0.25/10.83$ & $0.25/10.39$ & $0.26/9.93$ & $0.42/14.39$ & $0.54/11.17$ & 0.0 \\
  \midrule
  Uncertainty~\cite{kendall2018} & $0.19/9.32$ & $0.33/16.15$ & $0.30/17.86$ & $0.25/10.83$ & $0.25/11.22$ & $0.28/10.20$ & $0.48/14.60$ & $0.30/12.88$ & \color{teal}80.0 \\
  GradNorm~\cite{chen2018GradNorm} & $0.17/7.08$ & $0.33/13.54$ & $0.25/14.70$ & $0.24/9.65$ & $0.25/8.35$ & $0.26/9.08$ & $0.37/14.07$ & $0.27/10.92$ & \color{teal}100.00\\
  GradVac~\cite{wang2021gradvac} & $0.19/8.58$ & $0.32/13.21$ & $0.25/15.40$ & $0.24/10.86$ & $0.25/10.26$ & $0.27/10.30$ & $0.39/13.16$ & $0.27/11.68$ & \color{teal}100.00 \\
  MGDA~\cite{desideri2012MGDA} & $0.29/5.90$ & $0.73/11.84$ & $0.81/12.59$ & $0.33/8.67$ & $0.47/6.37$ & $0.33/9.08$ & $0.46/11.46$ & $0.49/9.42$ & \color{teal}10.20 \\
  MGDA-UB~\cite{sener2018MGDAUB} & $0.30/5.92$ & $0.73/11.74$ & $0.66/12.42$ & $0.59/9.09$ & $0.46/6.30$ & $0.57/8.69$ & $0.55/11.76$ & $0.55/9.42$ & \color{purple}-1.85 \\
  PCGrad~\cite{tianhe2020pcgrad} & $0.17/9.10$ & $0.30/13.17$ & $0.23/16.19$ & $0.23/10.57$ & $0.26/9.00$ & $0.25/10.35$ & $0.37/13.71$ & $0.26/11.73$ & \maxf{\color{teal}107.69} \\
  GradDrop~\cite{chen2020graddrop} & $0.20/11.60$ & $0.38/19.96$ & $0.34/24.59$ & $0.26/14.39$ & $0.27/14.69$ & $0.27/12.94$ & $0.37/20.39$ & $0.30/16.94$ & \color{teal}80.00 \\
  CAGrad~\cite{liu2021cagrad} & $0.17/6.01$ & $0.37/11.41$ & $0.33/12.72$ & $\maxf{0.24/8.05}$ & $0.26/6.58$ & $\maxf{0.27/8.50}$ & $0.47/12.59$ & $0.30/9.49$ & \color{teal}80.00 \\
  
  \midrule
  Aligned-MTL~(ours) & $0.18/5.82$ & $0.38/12.07$ & $0.49/18.15$ & $0.27/9.38$ & $0.34/8.99$ & $0.29/10.27$ & $0.41/12.84$ & $0.34/11.07$ & \color{teal}58.82 \\
  Aligned-MTL-UB~(ours) & $\maxf{0.16/5.40}$ & $\maxf{0.28/11.18}$ & $\maxf{0.23/12.14}$ & $0.28/9.57$ & $\maxf{0.24/6.17}$ & $0.27/8.51$ & $\maxf{0.35/11.54}$ & $0.26/9.22$ & \maxf{\color{teal}107.69}\\
  \bottomrule
\end{tabular}
\label{app:relocalization}
\end{table*}
